Unify Local and Global Information for Top-$N$ Recommendation

Knowledge graph (KG), integrating complex information and containing rich semantics, is widely considered as side information to enhance the recommendation systems. However, most of the existing KG-based methods concentrate on encoding the structural information in the graph, without utilizing the collaborative signals in user-item interaction data, which are important for understanding user preferences. Therefore, the representations learned by these models are insufficient for representing semantic information of users and items in the recommendation environment. The combination of both kinds of data provides a good chance to solve this problem. To tackle this research gap, we propose a novel duet representation learning framework named \sysname to fuse local information (user-item interaction data) and global information (external knowledge graph) for the top-$N$ recommendation, which is composed of two separate sub-models. One learns the local representations by discovering the inner correlations in local information with a knowledge-aware co-attention mechanism, and another learns the global representations by encoding the knowledge associations in global information with a relation-aware attention network. The two sub-models are jointly trained as part of the semantic fusion network to compute the user preferences, which discriminates the contribution of the two sub-models under the special context. We conduct experiments on two real-world datasets, and the evaluations show that KADM significantly outperforms state-of-art methods. Further ablation studies confirm that the duet architecture performs significantly better than either sub-model on the recommendation tasks.

==> body/rebuttal.tex <==
% % \clearpage
% \section*{Appendix}
% \appendix
% \fakeparagraph{Reviewer 1}

% Q1: Regarding KEE, the similarity coefficient for any item pair is computed as the proportion of users who interact with both items belonging to the pair. However, authors do not indicate a threshold for trusting on the similarity. For instance, if a user interacts with two items, and no other user has interacted with them, this similarity will be 1. Could a new threshold for weighting the similarities improve the results?

% A1: Thank you for asking this. Actually, we define their similarity coefficient as the proportion of users who interact with both items. If a user interacts with two items, and no other user has interacted with them, this similarity will be $\frac{1}{|\mathcal{U}|}$.

% Q2: Authors mention the resource and time consumption problems as a future work, but they do not report any (at least) preliminary result. However, it is an important concern for this work. In fact, authors make several decisions throughout the paper supported by computational efficiency. 

% A2: Thank you for asking this.  We have added a subsection (Sec. 4.5) to analyze the time complexity of \sysname.
% % As described in this paper, the enclosing subgraph extraction operation can greatly reduce the size of the graph, and only part of the relevant paths are preserved. 
% % And the subsequent computations are performed on a smaller-scale subgraph, which naturally improves computational efficiency.
% % Thus, the inference cost of KADM depends largely on the size of the extracted subgraphs, and the runtime in practice is usually dominated by running Dijkstras algorithm on these subgraphs.

% Q3: In the introduction and the related work sections authors claim that traditional CF methods suffer from the sparsity and cold-start problems and knowledge graphs try to incorporate new information for dealing with those problems. However, in the dataset description, authors set no threshold for Last.FM due to the sparsity issue. Why not to study the framework proposed in such a sparse scenario? 

% A3: Thank you for asking this.
% The reason for setting no threshold for Last.FM is that it is already a dataset in a sparse scenario.
% Setting a threshold will make it extremely sparse, which is another application scenario and other baselines in this scenario are not applicable. 
% Under this condition, we can not make effective comparisons between all methods.


% \fakeparagraph{Reviewer 2}

% Q1: The authors summarized several common limitations of existing KG-based recommendation methods. However, the proposed solutions for alleviating these limitations are not new. Especially, adopting an attention mechanism to avoid the negative noise from irrelevant entities and assign different weights for information from different relation paths is quite common.  

% A1: Thank you for pointing this out.
% In fact, The main limitations of existing KG-based methods are the efficiency problem brought by their computation on large-scale graphs and the noise introduced by the information propagation.
% And for avoiding the negative noise from irrelevant entities, we mainly filter out irrelevant noisy nodes by extracting the enclosing subgraph for the given user-item pair.
% As for assigning different weights to information from different relational paths, we actually use the weight calculation method obtained by improving the idea of R-GCN \cite{schlichtkrull2018modeling}, which has been explained in Section 4.3.

% Q2: Some closely related references are missing, such as the most recent KGIN and CKGAT. 

% A2: Thank you for the suggestion. We have added KGIN and CKGAT to the references.
% % For the two kinds of approaches, the main ideas of them are similar with KGAT \cite{wang2019kgat}. Therefore, they may have the same advantages and limitations. 
% % In this paper, we have already performed an exhaustive analysis of KGAT \cite{wang2019kgat}, so we do not repeat the introduction of these two methods.

% Q3: KGIN is the most recent KG-based recommendation method. It is better to compare with it in experiments.

% A3: Thank you for asking this.
% Actually, the interaction data is too sparse in our experimental environment. 
% As a result, KGIN cannot achieve a good effect.
% And the related implementation of KGIN is slightly different from the content described in the paper, which makes it difficult to get a suitable comparison result.
% So we removed this method during the comparative experiment.


% \fakeparagraph{Reviewer 3}

% Q1: If we do this on larger networks, say millions of nodes and edges, what does the performance look like? How scalable is the model? Do the authors have any insights on this?

% A1: Thank you for asking this.
% As described in this paper, for each user-item pair, we first extract the enclosing subgraph in the global model and perform subsequent operations on it. 
% Therefore, the scale of the original KG data does not affect the prediction process, but possible the efficiency of sub-graph extraction.

% Q2: It would be interesting to see the impacts of various characteristics of data on the results. For instance, if the user-item interaction is super sparse, or if the KG is sparse, how would that influence the accuracy of the recommendations?

% A2: Thank you for asking this. 
% This is a very interesting question.
% In fact, some of them have been discussed in this paper, such as when one of the user-item interaction data or the KG (extracted subgraph) data is extremely sparse, they can complement each other to achieve better recommendations.
% However, for the extreme case where both are sparse, there may not be a particularly obvious improvement in the recommendation performance.
% In response to this situation, our future research may try to add more auxiliary information or improve the model architecture to solve it.

% Q3: Will the codes be released?

% A3:Thank you for asking this. 
% We have added the codes links for this paper.
% %At present, the code and data are being sorted out, and the relevant content will be open sourced in time after completion. 
% Thank you for your interest in our work.
